Towards a global phase diagram of Ce-based dipolar-octupolar pyrochlore magnets under magnetic fields

Recent experiments have established a strong case for Ce$_2$(Zr, Sn, Hf)$_2$O$_7$ to host $\pi$-flux quantum spin ice (QSI). However, an irrefutable conclusion still requires strong, multifaceted evidence. In dipolar-octupolar (DO) compounds, external magnetic fields only strongly couple with the dipolar component $\tau_z$ along its local z-axis in contrast to octupolar components $\tau^{x,y}$. This gives rise to the unique ways magnetic fields interact with the system and, in turn, provides us with a variety of tuning knobs to generate comprehensive experimental results. In this work, we focus on magnetic fields along the (110), (111), and (001) directions and present a plethora of remarkable experimental signatures to probe the underlying physics of $\pi$-flux QSI using gauge mean field theory (GMFT) and Monte Carlo simulations. In particular, we present unique signatures in magnetic field-dependent phase diagrams, equal-time and dynamical structure factors, and magnetostriction.

==> xx.tex <==


